Stepwise Reasoning Verification: Don't Generate, Classify!

Verifying the reasoning of large language models is increasingly important as they are applied to complex mathematical and scientific problems. Existing work focuses on large decoder models and reports mixed results for generative and discriminative verifiers, leaving unclear which paradigm is more effective and whether large models are necessary. In this work, we cast stepwise verification as a natural language inference task: the problem and partial solution prefix form the premise, while the next reasoning step serves as the hypothesis to be classified as entailed or non-entailed. This formulation enables error localisation at individual reasoning steps and direct comparison of encoder classification, decoder classification, and decoder verdict generation across model scales and annotation budgets. Across five reasoning datasets, a 0.15B encoder classifier outperforms most generative verifiers with up to 4B parameters. On identical decoder backbones, classification outperforms generation from 0.5B to 4B parameters and matches it on the strongest 7B backbone---reaching comparable performance with roughly one tenth as many annotated problems. Our findings establish classification as a parameter- and data-efficient approach to stepwise verification and show that strong verification does not require large generative decoders.

==> sections/conclusion_legacy.tex <==
\section{Conclusion}
\label{sec:conclusion}

% \par We cast stepwise verification as local NLI and compared encoder classification, decoder classification, and decoder verdict generation on the same instances. On the same backbone, classification outperforms verdict generation at small scale and, at a practical verifier scale (Qwen2.5-3B), needs about ten times fewer annotated problems, and ties it on Qwen2.5-Math-7B; a 0.15B encoder classifier is competitive with generation decoders up to 4B. Initialising the classification head from the verdict tokens makes this reliable, so future comparisons of verification paradigms should control for head initialisation, and compact classifiers are a sound default for step-level verification.

\par Holding the backbone, instances, and prompt fixed isolates the training objective, and generating the verdict was no better than classifying it. The generative objective alone therefore does not account for the advantages reported for generative verifiers; these must come from what the objective is combined with, such as rationales, test-time sampling, or scale, none of which our controlled setting includes. Paradigm comparisons also depend on the benchmark: the gap between objectives is large on datasets where generation is weak and vanishes where both objectives saturate, so a comparison on a single dataset can report either, and benchmarks should be chosen with headroom. Testing rationale-generating verifiers under the same controls, and scales beyond 7B, is the next step.


==> tabs/cf_examples_tab.tex <==
\begin{table*}[htbp]
    \centering
    \begingroup
    \footnotesize
    \renewcommand{\arraystretch}{1.15}
    \begin{tabularx}{\textwidth}{
        @{}
        >{\raggedright\arraybackslash}p{1.55cm}
        >{\raggedright\arraybackslash}X
        >{\raggedright\arraybackslash}p{3.0cm}
        >{\raggedright\arraybackslash}X
        @{}
    }
        \toprule
        \textbf{Step ID}
        & \textbf{Original Step}
        & \textbf{Counterfactual Edit}
        & \textbf{Counterfactual Step} \\
        \midrule

        \texttt{13828-7}
        &
        Ok let's set $A$ at the origin and let $B$ be on the positive
        $x$-axis. \mbox{$(y_{\mathrm{orig}}=0)$}
        &
        Flip the orientation by placing $B$ on the negative $x$-axis.
        &
        Ok let's set $A$ at the origin and let $B$ be on the
        \textbf{negative} $x$-axis. \mbox{$(y_{\mathrm{cf}}=1)$}
        \\[2pt]

        \texttt{8323-53}
        &
        The heights of the two cones are
        $\frac{7\sqrt{10}}{4}-\frac{7}{\sqrt{10}}$
        and $\frac{7}{\sqrt{10}}$.
        \mbox{$(y_{\mathrm{orig}}=1)$}
        &
        Correct the arithmetic expressions derived from the geometric
        relations.
        &
        The heights of the two cones are
        $\frac{7\sqrt{10}}{4}
        -\mathbf{\frac{7}{2\sqrt{10}}}$
        and $\mathbf{\frac{7}{2\sqrt{10}}}$.
        \mbox{$(y_{\mathrm{cf}}=0)$}
        \\[2pt]

        \texttt{1769-13}
        &
        \ldots gives
        $x=\tan\!\left(
        \frac{1}{2}
        \left(\pi-\arcsin\frac{1}{3}\right)
        +k\pi
        \right)$.
        \mbox{$(y_{\mathrm{orig}}=0)$}
        &
        Remove the factor $\frac{1}{2}$ to introduce a common algebraic
        error.
        &
        \ldots gives
        $x=\tan\!\left(
        \mathbf{\left(\pi-\arcsin\frac{1}{3}\right)}
        +k\pi
        \right)$.
        \mbox{$(y_{\mathrm{cf}}=1)$}
        \\

        \bottomrule
    \end{tabularx}
    \endgroup

    \caption{\textbf{Qualitative examples of manually inspected counterfactual reasoning steps.} The counterfactual edit describes the targeted modification applied to each original step, and boldface highlights the corresponding textual or mathematical change in the generated counterfactual.}
    \label{tab:counterfactual_examples}
\end{table*}

==> tabs/config_tab.tex <==
\begin{table}[htbp]
    \centering
    \begingroup
    \setlength{\tabcolsep}{3.2pt}
    \renewcommand{\arraystretch}{1.08}
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{@{}lccc@{}}
        \toprule
        \textbf{Configuration}
        & \textbf{Encoder}
        & \textbf{Decoder-gen.}
        & \textbf{Decoder-cls.} \\
        \midrule
        Epochs                    & 5 (1)                  & 1 (0.5)             & 1 (0.5) \\
        Learning rate             & $1$--$2\times10^{-5}$ & $2\times10^{-5}$    & $2\times10^{-5}$ \\
        Scheduler                 & Cosine                 & Cosine               & Cosine \\
        Warmup ratio              & 0.10 (0.02)            & 0.10                 & 0.10 \\
        Weight decay              & 0.01                   & 0.01                 & 0.01 \\
        Maximum length            & 512 / 2,048            & 2,048                & 2,048 \\
        Gradient clipping         & 1.0                    & 1.0                  & 1.0 \\
        Checkpoint                & Best val.\ AUC         & Final                & Final \\
        \bottomrule
    \end{tabular}
    }
    \endgroup
    \caption{\textbf{Training configurations.} Parenthesised values apply to MathShepherd. Encoder learning rates and maximum lengths vary by backbone. All conditions use 8-bit AdamW, gradient clipping at 1.0, and seeds 1, 42, and 3407.}
    \label{tab:training_config}
\end{table}


==> tabs/counterfactual_tab.tex <==
\begin{table}[t]
    \centering
    \small
    \setlength{\tabcolsep}{5pt}
    \renewcommand{\arraystretch}{1.08}
    \begin{tabular}{@{}lcccc@{}}
        \toprule
        & \multicolumn{2}{c}{\textbf{CF AUC}}
        & \multicolumn{2}{c}{\textbf{ID AUC}} \\
        \cmidrule(lr){2-3}
        \cmidrule(lr){4-5}
        \textbf{Model}
        & \textbf{Original} & \textbf{DFR}
        & \textbf{Original} & \textbf{DFR} \\
        \midrule
        \multicolumn{5}{@{}l}{\textit{Encoders}} \\
        ModernBERT-B
        & .257 & .465
        & .779 & .579 \\
        ModernBERT-L
        & .272 & .423
        & .781 & .654 \\
        \addlinespace[2pt]
        \multicolumn{5}{@{}l}{\textit{Decoders (generation)}} \\
        Qwen2.5-0.5B
        & .340 & .466
        & .637 & .545 \\
        Qwen2.5-1.5B
        & .230 & .481
        & .709 & .573 \\
        Qwen2.5-3B
        & .357 & .645
        & .834 & .745 \\
        \addlinespace[2pt]
        \multicolumn{5}{@{}l}{\textit{Decoders (classification)}} \\
        Qwen2.5-0.5B
        & .247 & .433
        & .802 & .601 \\
        Qwen2.5-1.5B
        & .242 & .527
        & .826 & .640 \\
        Qwen2.5-3B
        & .267 & .647
        & .862 & .708 \\
        \bottomrule
    \end{tabular}
    \caption{\textbf{Linear feature reweighting partially recovers counterfactual discrimination at the cost of in-distribution performance.} DFR improves counterfactual AUC for every verifier, while in-distribution AUC decreases for every model.}
    \label{tab:cf_dfr}
\end{table}


==> tabs/loc_acc_results_tab.tex <==
\begin{table*}[t]
    \centering
    \small
    \setlength{\tabcolsep}{5pt}
    
    \begin{tabular}{l c *{5}{c} c c}
    \toprule
    \textbf{Model}
    & \textbf{Paradigm}
    & \textbf{PRM}
    & \textbf{MS}
    & \textbf{Epic}
    & \textbf{FoVer}
    & \textbf{MMLU}
    & \textbf{Avg.}
    & $\boldsymbol{\Delta}$ \\
    \midrule
    
    \multicolumn{9}{l}{\textit{Decoders}} \\
    
    \multirow{2}{*}{Qwen2.5-0.5B}
    & Gen.
    & \res{.449}{.030}
    & \res{.798}{.013}
    & \res{.966}{.013}
    & \res{.839}{.008}
    & \res{.680}{.015}
    & \res{.746}{.016}
    & \multirow{2}{*}{+.029} \\
    
    & Cls.
    & \res{.500}{.159}
    & \res{.811}{.026}
    & \res{.979}{.002}
    & \res{.884}{.031}
    & \res{.702}{.010}
    & \res{.775}{.046}
    & \\
    
    \addlinespace[3pt]
    
    \multirow{2}{*}{Qwen2.5-1.5B}
    & Gen.
    & \res{.490}{.157}
    & \res{.706}{.043}
    & \res{.961}{.015}
    & \res{.814}{.019}
    & \res{.728}{.021}
    & \res{.740}{.051}
    & \multirow{2}{*}{\textbf{+.065}} \\
    
    & Cls.
    & \res{.591}{.076}
    & \res{.830}{.017}
    & \res{.983}{.003}
    & \res{.891}{.086}
    & \res{.731}{.011}
    & \res{.805}{.039}
    & \\
    
    \addlinespace[3pt]
    
    \multirow{2}{*}{Qwen2.5-Math-1.5B}
    & Gen.
    & \res{.609}{.023}
    & \res{.821}{.008}
    & \res{.967}{.008}
    & \res{.878}{.014}
    & \res{.734}{.015}
    & \res{.802}{.014}
    & \multirow{2}{*}{+.042} \\
    
    & Cls.
    & \res{.653}{.116}
    & \res{.857}{.004}
    & \res{.983}{.003}
    & \res{.967}{.001}
    & \res{.761}{.005}
    & \res{.844}{.026}
    & \\
    
    \addlinespace[3pt]
    
    \multirow{2}{*}{Qwen2.5-3B}
    & Gen.
    & \res{.646}{.021}
    & \res{.812}{.007}
    & \res{.980}{.001}
    & \res{.890}{.033}
    & \res{.755}{.009}
    & \res{.817}{.014}
    & \multirow{2}{*}{+.021} \\
    
    & Cls.
    & \res{.680}{.010}
    & \res{.832}{.022}
    & \res{.980}{.005}
    & \res{.961}{.003}
    & \res{.738}{.067}
    & \res{.838}{.021}
    & \\
    
    \addlinespace[3pt]
    
    \multirow{2}{*}{Llama-3.2-3B}
    & Gen.
    & \res{.575}{.020}
    & \res{.799}{.057}
    & \res{.983}{.006}
    & \res{.876}{.005}
    & \res{.703}{.006}
    & \res{.787}{.019}
    & \multirow{2}{*}{+.027} \\
    
    & Cls.
    & \res{.605}{.003}
    & \res{.800}{.012}
    & \res{.980}{.003}
    & \res{.944}{.006}
    & \res{.738}{.009}
    & \res{.814}{.007}
    & \\
    
    \addlinespace[3pt]
    
    \multirow{2}{*}{Gemma-3-4B}
    & Gen.
    & \res{.413}{.175}
    & \res{.705}{.091}
    & \res{.954}{.001}
    & \res{.855}{.024}
    & \res{.713}{.030}
    & \res{.728}{.064}
    & \multirow{2}{*}{+.052} \\
    
    & Cls.
    & \res{.543}{.079}
    & \res{.810}{.014}
    & \res{.977}{.007}
    & \res{.879}{.042}
    & \res{.692}{.024}
    & \res{.780}{.033}
    & \\
    
    \addlinespace[3pt]
    
    \multirow{2}{*}{Qwen2.5-7B}
    & Gen.
    & \res{.720}{.016}
    & \res{.855}{.006}
    & \res{.984}{.001}
    & \res{.973}{.004}
    & \res{.794}{.007}
    & \res{.865}{.007}
    & \multirow{2}{*}{-.118} \\
    
    & Cls.
    & \res{.687}{.016}
    & \res{.852}{.005}
    & \res{.606}{.270}
    & \res{.890}{.057}
    & \res{.699}{.077}
    & \res{.747}{.085}
    & \\
    
    \addlinespace[3pt]
    
    \multirow{2}{*}{Qwen2.5-Math-7B}
    & Gen.
    & \res{\textbf{.776}}{.005}
    & \res{.866}{.005}
    & \res{.986}{.001}
    & \res{\textbf{.978}}{.001}
    & \res{.802}{.010}
    & \res{\textbf{.882}}{.004}
    & \multirow{2}{*}{-.001} \\
    
    & Cls.
    & \res{.761}{.007}
    & \res{.871}{.006}
    & \res{\textbf{.987}}{.002}
    & \res{.977}{.005}
    & \res{\textbf{.809}}{.003}
    & \res{.881}{.005}
    & \\
    
    \midrule
    
    \multicolumn{9}{l}{\textit{Encoders}} \\
    
    BERT-B (0.11B)
    & Cls.
    & \res{.527}{.021}
    & \res{.819}{.010}
    & \res{.531}{.023}
    & \res{.843}{.009}
    & \res{.664}{.014}
    & \res{.677}{.015}
    & \\
    
    BERT-L (0.34B)
    & Cls.
    & \res{.528}{.055}
    & \res{.845}{.028}
    & \res{.578}{.058}
    & \res{.793}{.057}
    & \res{.665}{.004}
    & \res{.682}{.040}
    & \\
    
    \addlinespace[2pt]
    
    RoBERTa-B (0.13B)
    & Cls.
    & \res{.582}{.024}
    & \res{.819}{.006}
    & \res{.979}{.001}
    & \res{.892}{.001}
    & \res{.647}{.020}
    & \res{.784}{.011}
    & \\
    
    RoBERTa-L (0.36B)
    & Cls.
    & \res{.559}{.024}
    & \res{.722}{.166}
    & \res{.976}{.003}
    & \res{.913}{.005}
    & \res{.647}{.023}
    & \res{.763}{.044}
    & \\
    
    \addlinespace[2pt]
    
    DeBERTa-B (0.18B)
    & Cls.
    & \res{.591}{.028}
    & \res{\textbf{.929}}{.057}
    & \res{.649}{.018}
    & \res{.903}{.002}
    & \res{.674}{.033}
    & \res{.749}{.027}
    & \\
    
    DeBERTa-L (0.44B)
    & Cls.
    & \res{.608}{.005}
    & \res{.845}{.032}
    & \res{.651}{.015}
    & \res{.918}{.009}
    & \res{.691}{.002}
    & \res{.743}{.013}
    & \\
    
    \addlinespace[2pt]
    
    ModernBERT-B (0.15B)
    & Cls.
    & \res{.603}{.042}
    & \res{.833}{.008}
    & \res{.986}{.001}
    & \res{.922}{.002}
    & \res{.678}{.028}
    & \res{{.805}{.016}
    & \\
    
    ModernBERT-L (0.4B)
    & Cls.
    & \res{.571}{.027}
    & \res{.788}{.054}
    & \res{.982}{.003}
    & \res{.932}{.015}
    & \res{.701}{.038}
    & \res{.795}{.028}
    & \\
    
    % \midrule
    
    % \multicolumn{9}{l}{\textit{Content-blind baselines}} \\
    
    % Random
    % &
    % & .274
    % & .645
    % & .295
    % & .555
    % & .276
    % & .409
    % & \\
    
    % Always Non-entailment
    % &
    % & .068
    % & .452
    % & .088
    % & .296
    % & .057
    % & .192
    % & \\
    
    % Position Prior
    % &
    % & .426
    % & .452
    % & .459
    % & .296
    % & .348
    % & .396
    % & \\
    
    % Length LR
    % &
    % & .357
    % & .709
    % & .290
    % & .739
    % & .309
    % & .481
    % & \\
    
    \bottomrule
    \end{tabular}
    
    \caption{
    \textbf{Conditional first-error ranking accuracy largely mirrors the step-level AUC results.}
    For each trajectory containing an annotated error, we select the step with the highest non-entailment score, $\hat{k}=\operatorname*{arg\,max}_i p_i$, and report whether it matches the annotated first-error position.
    Results are mean $\pm$ standard deviation over three random seeds.
    Bold marks the best result in each column among trained models. $\Delta$ denotes the difference in average accuracy, classification minus generation.}
    \label{tab:ranking_results}
\end{table*}


==> tabs/probe_tab.tex <==
% \begin{table*}[t]
%     \centering
%     \scriptsize
%     \setlength{\tabcolsep}{3pt}
%     \begin{minipage}[t]{0.49\textwidth}
%         \centering
%         \begin{tabular}{@{}rccc@{}}
%             \toprule
%             \textbf{Layer} & \textbf{Pretrained} & \textbf{Gen.\ SFT} & \textbf{Cls.\ FT} \\
%             \midrule
%             0 & $.545 \pm .026$ & $.548 \pm .027$ & $.541 \pm .026$ \\
%             1 & $.645 \pm .052$ & $.647 \pm .049$ & $.648 \pm .052$ \\
%             2 & $.647 \pm .032$ & $.648 \pm .038$ & $.650 \pm .030$ \\
%             3 & $.663 \pm .023$ & $.665 \pm .029$ & $.669 \pm .024$ \\
%             4 & $.667 \pm .038$ & $.673 \pm .040$ & $.664 \pm .028$ \\
%             5 & $.670 \pm .007$ & $.667 \pm .001$ & $.682 \pm .007$ \\
%             6 & $.668 \pm .011$ & $.666 \pm .010$ & $.681 \pm .014$ \\
%             7 & $.653 \pm .021$ & $.651 \pm .011$ & $.656 \pm .018$ \\
%             8 & $.682 \pm .038$ & $.678 \pm .042$ & $.684 \pm .036$ \\
%             9 & $.678 \pm .030$ & $.678 \pm .030$ & $.682 \pm .021$ \\
%             10 & $.680 \pm .023$ & $.682 \pm .017$ & $.681 \pm .024$ \\
%             11 & $.676 \pm .020$ & $.690 \pm .021$ & $.679 \pm .009$ \\
%             12 & $.662 \pm .027$ & $.657 \pm .029$ & $.673 \pm .022$ \\
%             13 & $.701 \pm .028$ & $.697 \pm .041$ & $.719 \pm .007$ \\
%             14 & $.676 \pm .013$ & $.686 \pm .013$ & $.685 \pm .015$ \\
%             15 & $.655 \pm .021$ & $.647 \pm .010$ & $.698 \pm .007$ \\
%             16 & $.697 \pm .008$ & $.699 \pm .013$ & $.693 \pm .019$ \\
%             17 & $.686 \pm .003$ & $.696 \pm .012$ & $.675 \pm .016$ \\
%             18 & $.668 \pm .020$ & $.674 \pm .026$ & $.706 \pm .016$ \\
%             \bottomrule
%         \end{tabular}
%     \end{minipage}
%     \hfill
%     \begin{minipage}[t]{0.49\textwidth}
%         \centering
%         \begin{tabular}{@{}rccc@{}}
%             \toprule
%             \textbf{Layer} & \textbf{Pretrained} & \textbf{Gen.\ SFT} & \textbf{Cls.\ FT} \\
%             \midrule
%             19 & $.671 \pm .017$ & $.686 \pm .014$ & $.707 \pm .036$ \\
%             20 & $.681 \pm .011$ & $.692 \pm .026$ & $.730 \pm .009$ \\
%             21 & $.722 \pm .015$ & $.716 \pm .024$ & $.765 \pm .043$ \\
%             22 & $.702 \pm .021$ & $.689 \pm .030$ & $.754 \pm .017$ \\
%             23 & $.712 \pm .018$ & $.701 \pm .032$ & $.795 \pm .009$ \\
%             24 & $.709 \pm .014$ & $.708 \pm .025$ & $.837 \pm .005$ \\
%             25 & $.698 \pm .013$ & $.710 \pm .022$ & $.885 \pm .008$ \\
%             26 & $.702 \pm .034$ & $.714 \pm .028$ & $.903 \pm .017$ \\
%             27 & $.703 \pm .003$ & $.707 \pm .043$ & $.914 \pm .013$ \\
%             28 & $.717 \pm .015$ & $.700 \pm .024$ & $.914 \pm .008$ \\
%             29 & $.724 \pm .026$ & $.728 \pm .006$ & $.917 \pm .013$ \\
%             30 & $.692 \pm .031$ & $.694 \pm .026$ & $.916 \pm .018$ \\
%             31 & $.687 \pm .017$ & $.712 \pm .012$ & $.923 \pm .009$ \\
%             32 & $.698 \pm .038$ & $.713 \pm .008$ & $.923 \pm .004$ \\
%             33 & $.713 \pm .012$ & $.735 \pm .029$ & $.923 \pm .003$ \\
%             34 & $.723 \pm .011$ & $.751 \pm .018$ & $.928 \pm .002$ \\
%             35 & $.715 \pm .012$ & $.733 \pm .037$ & $.929 \pm .008$ \\
%             36 & $.721 \pm .012$ & $.725 \pm .028$ & $.932 \pm .012$ \\
%             \bottomrule
%         \end{tabular}
%     \end{minipage}
%     \caption{\textbf{Layer-wise probing on PRM800K.} Each entry is validation AUC, reported as the mean and sample standard deviation over experiment seeds 1, 42, and 3407. Layer 0 is the embedding output and layers 1--36 are transformer-block outputs. }
%     \label{tab:probe_summary}
% \end{table*}

